Linking stellar populations to HII regions across nearby galaxies: I. Constraining pre-supernova feedback from young clusters in NGC1672

One of the fundamental factors regulating the evolution of galaxies is stellar feedback. However, we still do not have strong observational constraints on the relative importance of the different feedback mechanisms (e.g. radiation, ionised gas pressure, stellar winds) in driving HII region evolution and molecular cloud disruption. In this letter, we constrain the relative importance of the various feedback mechanisms from young massive star populations by resolving HII regions across the disk of the nearby star-forming galaxy NGC 1672. We combine measurements of ionised gas nebular lines obtained by PHANGS-MUSE, with high-resolution imaging from the HST in both the narrow-band H{\alpha} and broad-band filters. We identify a sample of 40 isolated, compact HII regions in the HST H{\alpha} image, for which we measure the sizes that were previously unresolved in seeing-limited ground-based observations. Additionally, we identify the ionisation source(s) for each HII region from catalogues produced as part of the PHANGS-HST survey. We find that the HII regions investigated are mildly dominated by thermal or wind pressure, yet their elevation above the radiation pressure is within the expected uncertainty range. We see that radiation pressure provides a substantially higher contribution to the total pressure than previously found in the literature over similar size scales. In general, we find higher pressures within more compact HII regions, which is driven by the inherent size scaling relations of each pressure term, albeit with significant scatter introduced by the variation in the stellar population properties (e.g. luminosity, mass, age, metallicity). For nearby galaxies, here we provide a promising approach that could yield the statistics required to map out how the importance of different stellar feedback mechanisms evolve over the lifetime of an HII region.

==> Paper - HST 1 - NGC1672 feedback (2)/authorlist.tex <==
%%%%% Please sign your name and affiliation below - in the format provided


%%% e.g. 
A. T. Barnes - Argelander-Institut f\"ur Astronomie, Universit\"at Bonn, Auf dem H\"ugel 71, 53121 Bonn, Germany 

%%% Please complete below.. 

L. Ubeda - Space Telescope Science Institute, Baltimore, MD 21218, USA 
B. Groves - International Centre for Radio Astronomy Research, The University of Western Australia, 35 Stirling Hwy, 6009 Crawley, WA, Australia
J.C. Lee - Gemini Observatory/NSF’s NOIRLab, 950 N. Cherry Avenue, Tucson, AZ, 85719, USA &
Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721
Francesco Belfiore, INAF— Osservatorio Astrofisico di Arcetri, Largo E. Fermi 5, I-50125, Florence, Italy
Médéric Boquien - Centro de Astronomía (CITEVA), Universidad de Antofagasta, Avenida Angamos 601, Antofagasta, Chile
Daniel A. Dale - Department of Physics \& Astronomy, University of Wyoming, Laramie, WY 82071 USA
Ralf S. Klessen - Universit\"at Heidelberg, Zentrum f\"ur Astronomie, Institut f\"ur Theoretische Astrophysik, Albert-Ueberle-Str.\ 2, 69120 Heidelberg, Germany  \& niversit\"{a}t Heidelberg, Interdisziplin\"{a}res Zentrum f\"{u}r Wissenschaftliches Rechnen, Im Neuenheimer Feld 225, 69120 Heidelberg, Germany
Adam K. Leroy - Department of Astronomy, The Ohio State University, 140 West 18th Avenue, Columbus, OH 43210, USA
Hsi-An Pan - Department of Physics, Tamkang University, No.151, Yingzhuan Road, Tamsui District, New Taipei City 251301, Taiwan
Thomas G. Williams - Max-Planck-Institut f\"{u}r Astronomie, K\"{o}nigstuhl 17, D-69117, Heidelberg, Germany
Enrico Congiu - Departamento de Astronoḿıa, Universidad de Chile, Camino del Observatorio 1515, Las Condes, Santiago, Chile
K. Grasha - ARC DECRA Fellow \& 
Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT 2611, Australia \&
ARC Centre of Excellence for All Sky Astrophysics in 3 Dimensions (ASTRO 3D), Australia   

Mattia C. Sormani - Universit\"{a}t Heidelberg, Zentrum f\"{u}r Astronomie, Institut f\"{u}r theoretische Astrophysik, Albert-Ueberle-Str. 2, 69120 Heidelberg, Germany

Cosima Eibensteiner - Argelander-Institut f\"ur Astronomie, Universit\"at Bonn, Auf dem H\"ugel 71, 53121 Bonn, Germany

Jakob den Brok - Argelander-Institut f\"ur Astronomie, Universit\"at Bonn, Auf dem H\"ugel 71, 53121 Bonn, Germany

J.~M.~Diederik Kruijssen - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, 69120 Heidelberg, Germany

Fabian Scheuermann - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, 69120 Heidelberg, Germany

Eric Emsellem - European Southern Observatory, Karl-Schwarzschild-Stra{\ss}e 2, 85748 Garching, Germany / Univ Lyon, Univ Lyon1, ENS de Lyon, CNRS, Centre de Recherche Astrophysique de Lyon UMR5574, F-69230 Saint-Genis-Laval France

Laura A. Lopez - Department of Astronomy, The Ohio State University, 140 West 18th Avenue, Columbus, OH 43210, USA

Hamid Hassani - 4-183 CCIS, University of Alberta, Edmonton, Alberta, T6G 2E1,
Canada

Kathryn Kreckel - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, D-69120 Heidelberg, Germany

Elizabeth J. Watkins - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, 69120 Heidelberg, Germany

Sinan Deger - TAPIR, California Institute of Technology, Pasadena, CA 91125, USA

==> Paper - HST 1 - NGC1672 feedback (2)/authors.tex <==
%%%%
\newcommand{\aifa}{Argelander-Institut f\"{u}r Astronomie, Universit\"{a}t Bonn, Auf dem H\"{u}gel 71, 53121, Bonn, Germany}
\newcommand{\ita}{Institut f\"{u}r Theoretische Astrophysik, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, Albert-Ueberle-Str 2, D-69120 Heidelberg, Germany}
\newcommand{\ari}{Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, 69120 Heidelberg, Germany}
\newcommand{\princeton}{Department of Astrophysical Sciences, Princeton University, Princeton, NJ 08544 USA}
\newcommand{\arcetri}{INAF — Osservatorio Astrofisico di Arcetri, Largo E. Fermi 5, I-50125, Florence, Italy}
\newcommand{\mpe}{Max-Planck-Institut f{\"u}r extraterrestrische Physik, Giessenbachstra{\ss}e~1, D-85748 Garching, Germany}
\newcommand{\zah}{Universit\"{a}t Heidelberg, Zentrum f\"{u}r Astronomie, Albert-Ueberle-Str. 2, 69120 Heidelberg, Germany}
\newcommand{\eso}{European Southern Observatory, Karl-Schwarzschild-Stra{\ss}e 2, 85748 Garching, Germany}
\newcommand{\ljmu}{Astrophysics Research Institute, Liverpool John Moores University, 146 Brownlow Hill, Liverpool L3 5RF, UK}
\newcommand{\stern}{Sternberg Astronomical Institute, Lomonosov Moscow State University, Universitetsky pr. 13, 119234 Moscow, Russia}
\newcommand{\alberta}{Department of Physics, University of Alberta, Edmonton, AB T6G 2E1, Canada}
\newcommand{\ohio}{Department of Astronomy, The Ohio State University, 140 West 18th Avenue, Columbus, OH 43210, USA}
\newcommand{\wyoming}{Department of Physics \& Astronomy, University of Wyoming, Laramie, WY 82071}
\newcommand{\mpia}{Max-Planck-Institute for Astronomy, K\"onigstuhl 17, D-69117 Heidelberg, Germany}
\newcommand{\iwr}{Universit\"{a}t Heidelberg, Interdisziplin\"{a}res Zentrum f\"{u}r Wissenschaftliches Rechnen, 69120 Heidelberg, Germany}
\newcommand{\anu}{Research School of Astronomy and Astrophysics, Australian National University, Weston Creek, ACT 2611, Australia}
\newcommand{\Nihon}{Department of Physics, General Studies, College of Engineering, Nihon University, 1 Nakagawara, Tokusada, Tamuramachi, Koriyama, Fukushima, 963-8642, Japan} 
\newcommand{\naoj}{National Astronomical Observatory of Japan, 2-21-1 Osawa, Mitaka, Tokyo, 181-8588, Japan} 
\newcommand{\usyd}{Sydney Institute for Astronomy, School of Physics, Physics Road, The University of Sydney, Darlington 2006, NSW, Australia} 
\newcommand{\UGent}{Sterrenkundig Observatorium, Universiteit Gent, Krijgslaan 281 S9, B-9000 Gent, Belgium}
\newcommand{\carnegie}{The Observatories of the Carnegie Institution for Science, 813 Santa Barbara Street, Pasadena, CA 91101, USA} 
\newcommand{\Uchile}{Departamento de Astronom\'ia, Universidad de Chile, Camino del Observatorio 1515, Las Condes, Santiago, Chile}
\newcommand{\nrao}{National Radio Astronomy Observatory, 520 Edgemont Road, Charlottesville, VA 22903, USA}
\newcommand{\UWaus}{International Centre for Radio Astronomy Research, University of Western Australia, 7 Fairway, Crawley, 6009, WA, Australia}
\newcommand{\UTol}{Ritter Astrophysical Research Center, The University of Toledo, Toledo, OH 43606, USA}
\newcommand{\CITEVA}{Centro de Astronom\'ia (CITEVA), Universidad de Antofagasta, Avenida Angamos 601, Antofagasta, Chile}
\newcommand{\UWyom}{Department of Physics \& Astronomy, University of Wyoming, Laramie, WY 82071 USA}
\newcommand{\leon}{Univ Lyon, ENS de Lyon, CNRS, Centre de Recherche Astrophysique de Lyon UMR5574, F-69230 Saint-Genis-Laval France}
\newcommand{\Gemini}{Gemini Observatory/NSF’s NOIRLab, 950 N. Cherry Avenue, Tucson, AZ, 85719, USA}
\newcommand{\Steward}{Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721}
\newcommand{\UTamkang}{Department of Physics, Tamkang University, No.151, Yingzhuan Road, Tamsui District, New Taipei City 251301, Taiwan}
\newcommand{\Umadrid}{Departamento de F\'isica Te\'orica, Universidad Autónoma de Madrid, 28049 Cantoblanco, Spain}
\newcommand{\stsci}{Space Telescope Science Institute, Baltimore, MD 21218, USA}
\newcommand{\Ucal}{Department of Physics \& Astronomy, University of California, Riverside, CA, USA}
\newcommand{\TAPIR}{TAPIR, California Institute of Technology, Pasadena, CA 91125, USA}
\newcommand{\UDurEA}{Centre for Extragalactic Astronomy, Department of Physics, Durham University, South Road, Durham DH1 3LE, UK}
\newcommand{\UDurCC}{Institute for Computational Cosmology, Department of Physics, University of Durham, South Road, Durham DH1 3LE, UK}
\newcommand{\JHop}{Department of Physics \& Astronomy, Bloomberg Center for Physics and Astronomy, Johns Hopkins University, 3400 N. Charles Street, Baltimore, MD 21218}
%%%%

\authorrunning{A.~T.~Barnes et al. }

\author{A.~T.~Barnes,\inst{1}\thanks{\url{ashleybarnes.astro@gmail.com}}
        R.~Chandar,\inst{2}
        K.~Kreckel,\inst{3}
        S.~C.~O.~Glover,\inst{4}
        F.~Scheuermann,\inst{3}
        F.~Belfiore,\inst{5}
        F.~Bigiel,\inst{1}
        G.~A.~Blanc,\inst{6,7}
        M.~Boquien,\inst{8}
        J.~den Brok,\inst{1}
        E.~Congiu,\inst{7}
        M.~Chevance,\inst{3}
        D.~A.~Dale,\inst{9}
        S.~Deger,\inst{10}
        J.~M.~D.~Kruijssen,\inst{3}
        O.~V.~Egorov,\inst{3}
        C.~Eibensteiner,\inst{1}
        E.~Emsellem,\inst{11,12}
        K.~Grasha,\inst{13}   
        B.~Groves,\inst{14} 
        R.~S.~Klessen,\inst{4,15} 
        S.~Hannon,\inst{16} 
        H.~Hassani,\inst{17} 
        J.~C.~Lee,\inst{18,19} 
        A.~K.~Leroy,\inst{20} 
        L.~A.~Lopez,\inst{20} 
        A.~F.~McLeod,\inst{21,22} 
        H.~Pan,\inst{23} 
        P.~S\'anchez-Bl\'azquez,\inst{24} 
        E.~Schinnerer,\inst{25} 
        M.~C.~Sormani,\inst{4}
        D.~A.~Thilker,\inst{26}
        L.~Ubeda,\inst{27} 
        E.~J.~Watkins,\inst{3}
        T.~G.~Williams\inst{25} 
        }

\institute{\aifa \and 
        \UTol \and
        \ari \and
        \ita \and 
        \arcetri \and
        \carnegie \and
        \Uchile \and
        \CITEVA \and
        \UWyom \and
        \TAPIR \and
        \eso \and
        \leon \and
        \anu \and
        \UWaus \and
        \iwr \and
        \Ucal \and
        \alberta \and
        \Gemini \and
        \Steward \and
        \ohio \and
        \UDurEA \and
        \UDurCC \and
        \UTamkang \and
        \Umadrid \and
        \mpia \and
        \JHop \and
        \stsci}

% K.~Kreckel - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, D-69120 Heidelberg, Germany
% S.~C.~O.~Glover - Institut f\"{u}r Theoretische Astrophysik, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, Albert-Ueberle-Str 2, D-69120 Heidelberg, Germany
% F.~Scheuermann - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, 69120 Heidelberg, Germany
% F.~Belfiore, INAF— Osservatorio Astrofisico di Arcetri, Largo E. Fermi 5, I-50125, Florence, Italy
% M.~Boquien - Centro de Astronomía (CITEVA), Universidad de Antofagasta, Avenida Angamos 601, Antofagasta, Chile
% J.~den Brok - Argelander-Institut f\"ur Astronomie, Universit\"at Bonn, Auf dem H\"ugel 71, 53121 Bonn, Germany
% E.~Congiu - Departamento de Astronoḿıa, Universidad de Chile, Camino del Observatorio 1515, Las Condes, Santiago, Chile
% M.~Chevance - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, 69120 Heidelberg, Germany 
% D.~A.~Dale - Department of Physics \& Astronomy, University of Wyoming, Laramie, WY 82071 USA
% J.~M.~Diederik Kruijssen - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, 69120 Heidelberg, Germany
% O.~Egorov - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, D-69120 Heidelberg, Germany
% C.~Eibensteiner - Argelander-Institut f\"ur Astronomie, Universit\"at Bonn, Auf dem H\"ugel 71, 53121 Bonn, Germany
% E.~Emsellem - European Southern Observatory, Karl-Schwarzschild-Stra{\ss}e 2, 85748 Garching, Germany / Univ Lyon, Univ Lyon1, ENS de Lyon, CNRS, Centre de Recherche Astrophysique de Lyon UMR5574, F-69230 Saint-Genis-Laval France
% K.~Grasha - Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT 2611, Australia \& ARC Centre of Excellence for All Sky Astrophysics in 3 Dimensions (ASTRO 3D), Australia   
% B.~Groves - International Centre for Radio Astronomy Research, The University of Western Australia, 35 Stirling Hwy, 6009 Crawley, WA, Australia
% R.~S.~Klessen - Universit\"at Heidelberg, Zentrum f\"ur Astronomie, Institut f\"ur Theoretische Astrophysik, Albert-Ueberle-Str.\ 2, 69120 Heidelberg, Germany  \& Universit\"{a}t Heidelberg, Interdisziplin\"{a}res Zentrum f\"{u}r Wissenschaftliches Rechnen, Im Neuenheimer Feld 225, 69120 Heidelberg, Germany
% H.~Hassani - 4-183 CCIS, University of Alberta, Edmonton, Alberta, T6G 2E1,Canada
% J.~C.~Lee - Gemini Observatory/NSF’s NOIRLab, 950 N. Cherry Avenue, Tucson, AZ, 85719, USA \& Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721
% A.~K.~Leroy - Department of Astronomy, The Ohio State University, 140 West 18th Avenue, Columbus, OH 43210, USA
% L.~A.~Lopez - Department of Astronomy, The Ohio State University, 140 West 18th Avenue, Columbus, OH 43210, USA
% H.~Pan - Department of Physics, Tamkang University, No.151, Yingzhuan Road, Tamsui District, New Taipei City 251301, Taiwan
% P.~Sa\'nchez-Bla\'zquez - Departamento de Física Teórica, Universidad Autónoma de Madrid, 28049 Cantoblanco, Spain
% M.~C.~Sormani - Universit\"{a}t Heidelberg, Zentrum f\"{u}r Astronomie, Institut f\"{u}r theoretische Astrophysik, Albert-Ueberle-Str. 2, 69120 Heidelberg, Germany
% L.~Ubeda - Space Telescope Science Institute, Baltimore, MD 21218, USA 
% T.~G.~Williams - Max-Planck-Institut f\"{u}r Astronomie, K\"{o}nigstuhl 17, D-69117, Heidelberg, Germany


==> Paper - HST 1 - NGC1672 feedback (2)/scratch/scratch.tex <==
%--------------------------------------------------- 
\begin{table}
    \centering
    \caption{Properties of the galaxy sample. We show in rows the galaxy name, central right ascension~(RA) and declination~(Dec), inclination~($i$), position angle~(PA), morphological type (Morph.), distance (Dist.), effective radius ($R_\mathrm{eff}$), globally averaged metallicity ($12+\log(\mathrm{O/H})$), total mass of atomic gas ($M_\mathrm{HI}$), molecular gas ($M_\mathrm{H_{2}}$) and stars ($M_\star$), and global star formation rate~(SFR).}
    \label{tab:galprops}
    
    \begin{tabular}{ccc}
    \hline
    Galaxy & Unit & Value \\
    \hline
    Name & - & NGC1672 \\ 
    RA $(a)$ & $\mathrm{{}^{\circ}}$ & 71.427 \\ 
    Dec $(a)$ & $\mathrm{{}^{\circ}}$ & -59.247 \\ 
    $i$ $(b)$ & $\mathrm{{}^{\circ}}$ & 42.6 \\
    PA $(b)$ & $\mathrm{{}^{\circ}}$ & 134.3 \\
    Morphology $(c)$ & - & Sb \\
    Distance $(d)$ & $\mathrm{Mpc}$ & 19.4 \\
    $R_\mathrm{eff}$ $(e)$ & $\mathrm{kpc}$ & 3.4 \\
    Metallicity $(f)$ & 12+log(O/H) & 8.56 \\
    $M_\mathrm{HI}$ $(g)$ & log($\mathrm{M_{\odot}}$) & 10.2 \\
    $M_\mathrm{H2}$ $(h)$ & log($\mathrm{M_{\odot}}$) & 9.9 \\
    $M_\star$ $(i)$ & log($\mathrm{M_{\odot}}$) & 10.7 \\
    SFR $(i)$ & log($\mathrm{M_{\odot}\,yr^{-1}}$) & 0.9\\
    \hline
    \end{tabular}

    \begin{minipage}{\columnwidth}
    \small
    \vspace{1mm} References: 
    $(a)$ From \cite{Salo2015}.
    $(b)$ From \cite{Lang2020}, based on PHANGS \mbox{CO(2--1)} kinematics. 
    $(c)$ Morphological classification taken from HyperLEDA \citep{Makarov2014}.
    $(d)$ Source distances are taken from the compilation of \citet{Anand2021}. 
    % $(d)$ Source distances are taken from several sources, using different methods. ic5332, ngc2835, ngc5068 are from PHANGSTRGB, using the Tip of the Red Giant Branch (TRGB) method. ngc0628, ngc1365, ngc3351, ngc3627, are from \citet{Jacobs2009} also using the TRGB method. ngc1433, ngc1512 are determined using the PNLF method from PHANGSPNLF. ngc1087, ngc1566, ngc4303 use the Group method and are from \citet{Kourkchi2017}. ngc1300, ngc1385, ngc1672, ngc7496 are determined using the NAM method from \citet{Shaya2017} and \citet{Kourkchi2020}. ngc4254 is determined using the SCM from \citet{Nugent2006}. ngc4321, ngc4535 are determine using Cepheids from \citet{Freedman2001}.  
    $(e)$ $R_\mathrm{eff}$ that contains half of the stellar mass of the galaxy \citep{Leroy2021a}. 
    $(f)$ Averaged metallicity within the area mapped by MUSE, computed using the Scal method of \citet{Pilyugin2016}; see \citet{kreckel19} for more details. 
    $(g)$ Total atomic gas mass taken from HYPERLEDA \citep{Makarov2014}.
    $(h)$ Total molecular gas mass determined from PHANGS \mbox{CO(2--1)} observations (see \citealp{Leroy2021a}). 
    $(i)$ Derived by \citet{Leroy2021a}, using \textit{GALEX}~UV and \textit{WISE}~IR photometry, following a similar methodology to \cite{Leroy2019}.
    \end{minipage}
      
\end{table}


==> Paper - HST 1 - NGC1672 feedback (2)/tables/table1.tex <==
\begin{sidewaystable*}
\caption{{\bf Properties of the \HII\ region sample.} We show in columns from left to right the ID, central RA and Dec, radius, galactocentric radius (normalised by the effective radius), extinction corrected \Ha\ flux, extinction, extinction corrected \Ha\ luminosity, metallicity, stellar population age and mass, bolometric and mechanical luminosity, mass loss rate, electron density, and thermal, radiation and wind pressures. A machine-readable version of this table is available online.}\label{tab1}
\centering
\begin{tabular}{ccccccccccccccccccc}
\hline\hline
ID & RA & Dec & $r$ & $R_\mathrm{gal}/R_\mathrm{eff}$ & $F_\mathrm{H\alpha,corr}$ & EBV & $L_\mathrm{H\alpha}$ & metal. & $t$ & $M$ & $L_\mathrm{bol}$ & $L_\mathrm{mech}$ & $\dot M$ & $n_\mathrm{e}$ & \ptherm & \pdir & \pwind \\
 & & & & & log$_{10}$() & & log$_{10}$() & & & log$_{10}$() & log$_{10}$() & log$_{10}$() & log$_{10}$() & & log$_{10}$() & log$_{10}$() & log$_{10}$() \\
 & $\mathrm{{}^{\circ}}$ & $\mathrm{{}^{\circ}}$ & $\mathrm{pc}$ &  & $\mathrm{erg\,s^{-1}\,cm^{-2}}$ & $\mathrm{mag}$ & $\mathrm{L_{\odot}}$ & 12+log(O/H) & $\mathrm{Myr}$ & $\mathrm{M_{\odot}}$ & $\mathrm{L_{\odot}}$ & $\mathrm{erg\,s^{-1}}$ & $\mathrm{g\,s^{-1}}$ & $\mathrm{cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ \\
 \hline
0 & 71.452 & -59.256 & 10.1 & 1.6 & -14.95 & 0.144 & 4.12 & 8.58 & 1 & 3.71 & 5.9 & 37.7 & 20.9 & 30.4 & 5.69 & 5.26 & 5.65 \\
1 & 71.400 & -59.260 & 12.9 & 2.58 & -14.93 & 0.277 & 4.14 & 8.56 & 2 & 3.49 & 5.99 & 37.4 & 20.6 & 21.8 & 5.54 & 5.14 & 5.23 \\
2 & 71.389 & -59.249 & 42.6 & 2.36 & -13.48 & 0.301 & 5.58 & 8.55 & 1 & 5 & 7.37 & 38.9 & 22.1 & 18.3 & 5.43 & 5.47 & 5.69 \\
3 & 71.476 & -59.232 & 20.6 & 3.94 & -13.84 & 0.248 & 5.23 & 8.56 & 1 & 4.3 & 7.01 & 38.2 & 21.4 & 36 & 5.71 & 5.75 & 5.62 \\
4 & 71.459 & -59.246 & 14.6 & 1.95 & -14.86 & 0.17 & 4.21 & 8.57 & 2 & 3.54 & 6.06 & 37.5 & 20.7 & 19.4 & 5.49 & 5.09 & 5.16 \\
5 & 71.437 & -59.245 & 22.7 & 0.752 & -14.47 & 0.3 & 4.59 & 8.61 & 4 & 3.52 & 6.8 & 37.5 & 20.7 & 15.7 & 5.4 & 5.46 & 4.75 \\
6 & 71.468 & -59.240 & 7.17 & 2.82 & -15.04 & 0.369 & 4.02 & 8.54 & 4 & 3.68 & 6.23 & 37.6 & 20.8 & 45.8 & 5.86 & 5.88 & 5.92 \\
7 & 71.483 & -59.234 & 15.3 & 4.13 & -14.46 & 0.185 & 4.61 & 8.52 & 1 & 3.93 & 6.4 & 37.9 & 21.1 & 28.8 & 5.66 & 5.39 & 5.51 \\
8 & 71.471 & -59.228 & 19.2 & 3.97 & -14.09 & 0.288 & 4.97 & 8.62 & 1 & 4.06 & 6.76 & 38 & 21.2 & 30.7 & 5.67 & 5.56 & 5.44 \\
9 & 71.428 & -59.236 & 9.99 & 1.42 & -14.69 & 0.22 & 4.38 & 8.58 & 1 & 3.8 & 6.16 & 37.7 & 20.9 & 41.9 & 5.83 & 5.53 & 5.76 \\
10 & 71.483 & -59.246 & 6.09 & 3.47 & -14.50 & 0.418 & 4.56 & 8.51 & 2 & 4.32 & 6.42 & 38.3 & 21.5 & 109 & 6.24 & 6.21 & 6.7 \\
11 & 71.380 & -59.250 & 4.74 & 2.93 & -14.79 & 0.358 & 4.27 & 8.58 & 1 & 3.65 & 6.06 & 37.6 & 20.8 & 114 & 6.26 & 6.07 & 6.25 \\
12 & 71.380 & -59.245 & 5.56 & 2.77 & -14.36 & 0.278 & 4.70 & 8.52 & 2 & 3.91 & 6.55 & 37.8 & 21.1 & 154 & 6.44 & 6.43 & 6.37 \\
13 & 71.376 & -59.240 & 11.3 & 2.96 & -14.90 & 0.296 & 4.17 & 8.58 & 1 & 3.95 & 5.95 & 37.9 & 21.1 & 31.8 & 5.86 & 5.21 & 5.8 \\
14 & 71.414 & -59.235 & 14.7 & 1.45 & -14.22 & 0.563 & 4.84 & 8.61 & 1 & 4.43 & 6.63 & 38.4 & 21.6 & 40.1 & 5.81 & 5.66 & 6.05 \\
15 & 71.374 & -59.251 & 8.26 & 3.36 & -14.83 & 0.238 & 4.24 & 8.54 & 1 & 3.64 & 6.02 & 37.6 & 20.8 & 47.4 & 5.88 & 5.55 & 5.75 \\
16 & 71.369 & -59.257 & 8.63 & 4.08 & -15.08 & 0.125 & 3.99 & 8.52 & 2 & 3.43 & 5.84 & 37.4 & 20.6 & 33.5 & 5.73 & 5.34 & 5.51 \\
17 & 71.385 & -59.241 & 12.5 & 2.45 & -14.09 & 0.35 & 4.97 & 8.54 & 1 & 4.17 & 6.76 & 38.1 & 21.3 & 58.8 & 5.96 & 5.93 & 5.93 \\
18 & 71.392 & -59.237 & 11.8 & 2.11 & -14.78 & 0.171 & 4.28 & 8.55 & 1 & 3.94 & 6.07 & 37.9 & 21.1 & 29.1 & 5.67 & 5.29 & 5.75 \\
19 & 71.375 & -59.250 & 19.2 & 3.3 & -13.66 & 0.308 & 5.41 & 8.51 & 2 & 4.17 & 7.26 & 38.1 & 21.3 & 53 & 5.95 & 6.06 & 5.55 \\
20 & 71.451 & -59.259 & 11.3 & 1.67 & -14.95 & 0.239 & 4.12 & 8.54 & 1 & 3.42 & 5.9 & 37.4 & 20.6 & 25.9 & 5.62 & 5.16 & 5.27 \\
21 & 71.480 & -59.243 & 7.41 & 3.4 & -15.03 & 0.205 & 4.04 & 8.50 & 1 & 3.68 & 5.82 & 37.6 & 20.8 & 44.5 & 5.85 & 5.45 & 5.89 \\
22 & 71.402 & -59.244 & 7.58 & 1.48 & -14.74 & 0.327 & 4.33 & 8.56 & 1 & 3.99 & 6.11 & 37.9 & 21.1 & 59.9 & 5.98 & 5.72 & 6.18 \\
23 & 71.379 & -59.243 & 5.97 & 2.81 & -15.21 & 0.233 & 3.86 & 8.54 & 1 & 3.37 & 5.64 & 37.3 & 20.5 & 49.8 & 5.9 & 5.45 & 5.77 \\
24 & 71.391 & -59.244 & 22.8 & 2.13 & -14.25 & 0.106 & 4.81 & 8.54 & 2 & 3.46 & 6.66 & 37.4 & 20.6 & 19.9 & 5.49 & 5.32 & 4.7 \\
25 & 71.421 & -59.241 & 9.12 & 0.727 & -15.18 & 0.259 & 3.88 & 8.59 & 2 & 3.3 & 5.73 & 37.2 & 20.4 & 27.1 & 5.64 & 5.18 & 5.32 \\
26 & 71.433 & -59.237 & 13.4 & 1.42 & -14.49 & 0.257 & 4.57 & 8.58 & 1 & 4.06 & 6.36 & 38 & 21.2 & 34 & 5.74 & 5.47 & 5.76 \\
27 & 71.395 & -59.240 & 11.2 & 1.89 & -15.10 & 0.144 & 3.97 & 8.56 & 1 & 3.75 & 5.76 & 37.7 & 20.9 & 22.1 & 5.55 & 5.02 & 5.6 \\
28 & 71.403 & -59.260 & 8.27 & 2.37 & -15.18 & 0.305 & 3.88 & 8.56 & 3 & 3.45 & 6.01 & 37.4 & 20.6 & 31.5 & 5.7 & 5.54 & 5.57 \\
29 & 71.454 & -59.256 & 8.07 & 1.68 & -14.96 & 0.131 & 4.11 & 8.54 & 2 & 3.6 & 5.96 & 37.5 & 20.7 & 42.4 & 5.83 & 5.51 & 5.74 \\
30 & 71.478 & -59.244 & 6.43 & 3.2 & -15.05 & 0.103 & 4.02 & 8.51 & 2 & 3.39 & 5.87 & 37.3 & 20.5 & 53.6 & 5.93 & 5.62 & 5.73 \\
31 & 71.469 & -59.227 & 6.22 & 3.98 & -14.88 & 0.264 & 4.19 & 8.59 & 1 & 3.93 & 5.97 & 37.9 & 21.1 & 68.4 & 6.04 & 5.75 & 6.29 \\
32 & 71.453 & -59.242 & 11.9 & 1.9 & -15.18 & 0.241 & 3.88 & 8.59 & 2 & 2.89 & 5.73 & 36.8 & 20 & 18.3 & 5.47 & 4.95 & 4.69 \\
33 & 71.418 & -59.256 & 12.5 & 1.36 & -15.01 & 0.194 & 4.05 & 8.59 & 4 & 3.03 & 6.26 & 37 & 20.2 & 20.5 & 5.52 & 5.43 & 4.78 \\
34 & 71.418 & -59.257 & 15 & 1.42 & -14.58 & 0.31 & 4.49 & 8.63 & 1 & 3.8 & 6.27 & 37.7 & 20.9 & 27 & 5.68 & 5.29 & 5.4 \\
35 & 71.408 & -59.261 & 19.7 & 2.23 & -14.52 & 0.249 & 4.55 & 8.55 & 2 & 3.7 & 6.4 & 37.6 & 20.8 & 18.5 & 5.47 & 5.18 & 5.06 \\
36 & 71.396 & -59.248 & 6.69 & 1.93 & -14.85 & 0.337 & 4.22 & 8.60 & 1 & 3.68 & 6 & 37.6 & 20.8 & 63.5 & 6.01 & 5.72 & 5.98 \\
37 & 71.416 & -59.255 & 15.9 & 1.29 & -14.15 & 0.387 & 4.92 & 8.60 & 1 & 4.32 & 6.7 & 38.3 & 21.5 & 40.3 & 5.85 & 5.67 & 5.87 \\
38 & 71.463 & -59.244 & 7.62 & 2.28 & -14.79 & 0.39 & 4.27 & 8.56 & 4 & 3.65 & 6.48 & 37.6 & 20.8 & 55.8 & 5.95 & 6.08 & 5.84 \\
39 & 71.451 & -59.251 & 8.59 & 1.38 & -15.03 & 0.166 & 4.03 & 8.59 & 2 & 3.32 & 5.88 & 37.3 & 20.5 & 35.4 & 5.75 & 5.38 & 5.4 \\
\hline\hline
\end{tabular}
\end{sidewaystable*}

% \begin{table}
% \centering
% \begin{tabular}{ccccccccccccc}
% \hline\hline
% id & ra & dec & $r_\mathrm{maj}$ & $r_\mathrm{min}$ & PA & $r$ & $R_\mathrm{gal}/R_\mathrm{eff}$ & $F_\mathrm{H\alpha}$ & $F_\mathrm{H\alpha,corr}$ & EBV & $L_\mathrm{H\alpha}$ & metal. \\
%  &  &  &  &  &  &  &  & log$_{10}$() & log$_{10}$() & & log$_{10}$() \\
%  & $\mathrm{{}^{\circ}}$ & $\mathrm{{}^{\circ}}$ & $\mathrm{{}^{\prime\prime}}$ & $\mathrm{{}^{\prime\prime}}$ & $\mathrm{{}^{\circ}}$ & $\mathrm{pc}$ &  & $\mathrm{erg\,s^{-1}\,cm^{-2}}$ & $\mathrm{erg\,s^{-1}\,cm^{-2}}$ & $\mathrm{mag}$ & $\mathrm{L_{\odot}}$ & 12+log(O/H)\\
%  \hline
% 0 & 71.452 & -59.256 & 0.11 & 0.11 & 76 & 10 & 1.6 & -15.09 & -14.95 & 0.14 & 4.12 & 8.58 \\
% 1 & 71.400 & -59.260 & 0.16 & 0.11 & 132 & 13 & 2.6 & -15.21 & -14.93 & 0.28 & 4.14 & 8.56 \\
% 3 & 71.389 & -59.249 & 0.47 & 0.44 & 129 & 43 & 2.4 & -13.78 & -13.48 & 0.3 & 5.58 & 8.55 \\
% 4 & 71.476 & -59.232 & 0.27 & 0.18 & 107 & 21 & 3.9 & -14.09 & -13.84 & 0.25 & 5.23 & 8.56 \\
% 6 & 71.459 & -59.246 & 0.16 & 0.15 & 166 & 15 & 2 & -15.03 & -14.86 & 0.17 & 4.21 & 8.57 \\
% 7 & 71.437 & -59.245 & 0.29 & 0.2 & 166 & 23 & 0.75 & -14.77 & -14.47 & 0.3 & 4.59 & 8.61 \\
% 9 & 71.468 & -59.240 & 0.091 & 0.064 & 131 & 7.2 & 2.8 & -15.42 & -15.04 & 0.37 & 4.02 & 8.54 \\
% 10 & 71.483 & -59.234 & 0.17 & 0.16 & 58 & 15 & 4.1 & -14.64 & -14.46 & 0.18 & 4.61 & 8.52 \\
% % 11 & 71.471 & -59.228 & 0.23 & 0.18 & 140 & 19 & 4 & -14.38 & -14.09 & 0.29 & 4.97 & 8.62 \\
% % 12 & 71.428 & -59.236 & 0.15 & 0.077 & 117 & 10 & 1.4 & -14.91 & -14.69 & 0.22 & 4.38 & 8.58 \\
% % 13 & 71.483 & -59.246 & 0.069 & 0.061 & 169 & 6.1 & 3.5 & -14.92 & -14.50 & 0.42 & 4.56 & 8.51 \\
% % 14 & 71.380 & -59.250 & 0.056 & 0.046 & 143 & 4.7 & 2.9 & -15.15 & -14.79 & 0.36 & 4.27 & 8.58 \\
% % 15 & 71.380 & -59.245 & 0.065 & 0.053 & 84 & 5.6 & 2.8 & -14.64 & -14.36 & 0.28 & 4.70 & 8.52 \\
% % 16 & 71.376 & -59.240 & 0.18 & 0.081 & 152 & 11 & 3 & -15.20 & -14.90 & 0.3 & 4.17 & 8.58 \\
% % 18 & 71.414 & -59.235 & 0.22 & 0.11 & 56 & 15 & 1.4 & -14.79 & -14.22 & 0.56 & 4.84 & 8.61 \\
% % 20 & 71.374 & -59.251 & 0.1 & 0.077 & 139 & 8.3 & 3.4 & -15.07 & -14.83 & 0.24 & 4.24 & 8.54 \\
% % 21 & 71.369 & -59.257 & 0.11 & 0.08 & 177 & 8.6 & 4.1 & -15.20 & -15.08 & 0.13 & 3.99 & 8.52 \\
% % 22 & 71.385 & -59.241 & 0.16 & 0.11 & 127 & 12 & 2.5 & -14.45 & -14.09 & 0.35 & 4.97 & 8.54 \\
% % 23 & 71.392 & -59.237 & 0.13 & 0.12 & 123 & 12 & 2.1 & -14.96 & -14.78 & 0.17 & 4.28 & 8.55 \\
% % 24 & 71.375 & -59.250 & 0.25 & 0.17 & 154 & 19 & 3.3 & -13.97 & -13.66 & 0.31 & 5.41 & 8.51 \\
% % 25 & 71.451 & -59.259 & 0.15 & 0.096 & 113 & 11 & 1.7 & -15.19 & -14.95 & 0.24 & 4.12 & 8.54 \\
% % 26 & 71.480 & -59.243 & 0.083 & 0.075 & 157 & 7.4 & 3.4 & -15.23 & -15.03 & 0.21 & 4.04 & 8.50 \\
% % 27 & 71.402 & -59.244 & 0.096 & 0.067 & 72 & 7.6 & 1.5 & -15.07 & -14.74 & 0.33 & 4.33 & 8.56 \\
% % 28 & 71.379 & -59.243 & 0.066 & 0.061 & -166 & 6 & 2.8 & -15.44 & -15.21 & 0.23 & 3.86 & 8.54 \\
% % 29 & 71.391 & -59.244 & 0.27 & 0.22 & -137 & 23 & 2.1 & -14.36 & -14.25 & 0.11 & 4.81 & 8.54 \\
% % 30 & 71.421 & -59.241 & 0.11 & 0.087 & -151 & 9.1 & 0.73 & -15.45 & -15.18 & 0.26 & 3.88 & 8.59 \\
% % 31 & 71.433 & -59.237 & 0.15 & 0.13 & 117 & 13 & 1.4 & -14.75 & -14.49 & 0.26 & 4.57 & 8.58 \\
% % 32 & 71.395 & -59.240 & 0.13 & 0.11 & 129 & 11 & 1.9 & -15.24 & -15.10 & 0.14 & 3.97 & 8.56 \\
% % 34 & 71.403 & -59.260 & 0.14 & 0.057 & 60 & 8.3 & 2.4 & -15.49 & -15.18 & 0.3 & 3.88 & 8.56 \\
% % 35 & 71.454 & -59.256 & 0.089 & 0.083 & -142 & 8.1 & 1.7 & -15.09 & -14.96 & 0.13 & 4.11 & 8.54 \\
% % 37 & 71.478 & -59.244 & 0.071 & 0.065 & 101 & 6.4 & 3.2 & -15.15 & -15.05 & 0.1 & 4.02 & 8.51 \\
% % 38 & 71.469 & -59.227 & 0.073 & 0.06 & 99 & 6.2 & 4 & -15.15 & -14.88 & 0.26 & 4.19 & 8.59 \\
% % 40 & 71.453 & -59.242 & 0.16 & 0.1 & 74 & 12 & 1.9 & -15.43 & -15.18 & 0.24 & 3.88 & 8.59 \\
% % 42 & 71.418 & -59.256 & 0.16 & 0.11 & -164 & 13 & 1.4 & -15.21 & -15.01 & 0.19 & 4.05 & 8.59 \\
% % 43 & 71.418 & -59.257 & 0.2 & 0.13 & 65 & 15 & 1.4 & -14.89 & -14.58 & 0.31 & 4.49 & 8.63 \\
% % 44 & 71.408 & -59.261 & 0.3 & 0.15 & 55 & 20 & 2.2 & -14.77 & -14.52 & 0.25 & 4.55 & 8.55 \\
% % 45 & 71.396 & -59.248 & 0.075 & 0.067 & 156 & 6.7 & 1.9 & -15.19 & -14.85 & 0.34 & 4.22 & 8.60 \\
% % 47 & 71.416 & -59.255 & 0.18 & 0.16 & 94 & 16 & 1.3 & -14.54 & -14.15 & 0.39 & 4.92 & 8.60 \\
% % 49 & 71.463 & -59.244 & 0.093 & 0.071 & 89 & 7.6 & 2.3 & -15.19 & -14.79 & 0.39 & 4.27 & 8.56 \\
% % 50 & 71.451 & -59.251 & 0.11 & 0.079 & 54 & 8.6 & 1.4 & -15.20 & -15.03 & 0.17 & 4.03 & 8.59 \\
% \hline\hline
% \end{tabular}
% \end{table}



% \begin{table}
% \begin{tabular}{ccccccccccc}
% \hline\hline
% id & $t$ & $M$ & $L_\mathrm{bol}$ & $L_\mathrm{mech}$ & $\dot M$ & $v_\mathrm{wind}$ & $n_\mathrm{e}$ & \ptherm & \pdir & \pwind \\
% & log$_{10}$() & log$_{10}$() & log$_{10}$() & log$_{10}$() & log$_{10}$() & log$_{10}$() & & log$_{10}$() & log$_{10}$() & log$_{10}$() \\
% & $\mathrm{Myr}$ & $\mathrm{M_{\odot}}$ & $\mathrm{L_{\odot}}$ & $\mathrm{erg\,s^{-1}}$ & $\mathrm{g\,s^{-1}}$ & $\mathrm{km\,s^{-1}}$ & $\mathrm{cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ \\
% \hline
% 0 & 6 & 3.71 & 5.9 & 37.7 & 20.9 & 3522 & 30.4 & 5.69 & 5.26 & 5.65 \\
% 1 & 6.3 & 3.49 & 5.99 & 37.4 & 20.6 & 3522 & 21.8 & 5.54 & 5.14 & 5.23 \\
% 3 & 6 & 5 & 7.37 & 38.9 & 22.1 & 3522 & 18.3 & 5.43 & 5.47 & 5.69 \\
% 4 & 6 & 4.3 & 7.01 & 38.2 & 21.4 & 3522 & 36 & 5.71 & 5.75 & 5.62 \\
% 6 & 6.3 & 3.54 & 6.06 & 37.5 & 20.7 & 3522 & 19.4 & 5.49 & 5.09 & 5.16 \\
% 7 & 6.6 & 3.52 & 6.8 & 37.5 & 20.7 & 3522 & 15.7 & 5.4 & 5.46 & 4.75 \\
% 9 & 6.6 & 3.68 & 6.23 & 37.6 & 20.8 & 3522 & 45.8 & 5.86 & 5.88 & 5.92 \\
% 10 & 6 & 3.93 & 6.4 & 37.9 & 21.1 & 3522 & 28.8 & 5.66 & 5.39 & 5.51 \\
% % 11 & 6 & 4.06 & 6.76 & 38 & 21.2 & 3522 & 30.7 & 5.67 & 5.56 & 5.44 \\
% % 12 & 6 & 3.8 & 6.16 & 37.7 & 20.9 & 3522 & 41.9 & 5.83 & 5.53 & 5.76 \\
% % 13 & 6.3 & 4.32 & 6.42 & 38.3 & 21.5 & 3522 & 109 & 6.24 & 6.21 & 6.7 \\
% % 14 & 6 & 3.65 & 6.06 & 37.6 & 20.8 & 3522 & 114 & 6.26 & 6.07 & 6.25 \\
% % 15 & 6.3 & 3.91 & 6.55 & 37.8 & 21.1 & 3522 & 154 & 6.44 & 6.43 & 6.37 \\
% % 16 & 6 & 3.95 & 5.95 & 37.9 & 21.1 & 3522 & 31.8 & 5.86 & 5.21 & 5.8 \\
% % 18 & 6 & 4.43 & 6.63 & 38.4 & 21.6 & 3522 & 40.1 & 5.81 & 5.66 & 6.05 \\
% % 20 & 6 & 3.64 & 6.02 & 37.6 & 20.8 & 3522 & 47.4 & 5.88 & 5.55 & 5.75 \\
% % 21 & 6.3 & 3.43 & 5.84 & 37.4 & 20.6 & 3522 & 33.5 & 5.73 & 5.34 & 5.51 \\
% % 22 & 6 & 4.17 & 6.76 & 38.1 & 21.3 & 3522 & 58.8 & 5.96 & 5.93 & 5.93 \\
% % 23 & 6 & 3.94 & 6.07 & 37.9 & 21.1 & 3522 & 29.1 & 5.67 & 5.29 & 5.75 \\
% % 24 & 6.3 & 4.17 & 7.26 & 38.1 & 21.3 & 3522 & 53 & 5.95 & 6.06 & 5.55 \\
% % 25 & 6 & 3.42 & 5.9 & 37.4 & 20.6 & 3522 & 25.9 & 5.62 & 5.16 & 5.27 \\
% % 26 & 6 & 3.68 & 5.82 & 37.6 & 20.8 & 3522 & 44.5 & 5.85 & 5.45 & 5.89 \\
% % 27 & 6 & 3.99 & 6.11 & 37.9 & 21.1 & 3522 & 59.9 & 5.98 & 5.72 & 6.18 \\
% % 28 & 6 & 3.37 & 5.64 & 37.3 & 20.5 & 3522 & 49.8 & 5.9 & 5.45 & 5.77 \\
% % 29 & 6.3 & 3.46 & 6.66 & 37.4 & 20.6 & 3522 & 19.9 & 5.49 & 5.32 & 4.7 \\
% % 30 & 6.3 & 3.3 & 5.73 & 37.2 & 20.4 & 3522 & 27.1 & 5.64 & 5.18 & 5.32 \\
% % 31 & 6 & 4.06 & 6.36 & 38 & 21.2 & 3522 & 34 & 5.74 & 5.47 & 5.76 \\
% % 32 & 6 & 3.75 & 5.76 & 37.7 & 20.9 & 3522 & 22.1 & 5.55 & 5.02 & 5.6 \\
% % 34 & 6.48 & 3.45 & 6.01 & 37.4 & 20.6 & 3522 & 31.5 & 5.7 & 5.54 & 5.57 \\
% % 35 & 6.3 & 3.6 & 5.96 & 37.5 & 20.7 & 3522 & 42.4 & 5.83 & 5.51 & 5.74 \\
% % 37 & 6.3 & 3.39 & 5.87 & 37.3 & 20.5 & 3522 & 53.6 & 5.93 & 5.62 & 5.73 \\
% % 38 & 6 & 3.93 & 5.97 & 37.9 & 21.1 & 3522 & 68.4 & 6.04 & 5.75 & 6.29 \\
% % 40 & 6.3 & 2.89 & 5.73 & 36.8 & 20 & 3522 & 18.3 & 5.47 & 4.95 & 4.69 \\
% % 42 & 6.6 & 3.03 & 6.26 & 37 & 20.2 & 3522 & 20.5 & 5.52 & 5.43 & 4.78 \\
% % 43 & 6 & 3.8 & 6.27 & 37.7 & 20.9 & 3522 & 27 & 5.68 & 5.29 & 5.4 \\
% % 44 & 6.3 & 3.7 & 6.4 & 37.6 & 20.8 & 3522 & 18.5 & 5.47 & 5.18 & 5.06 \\
% % 45 & 6 & 3.68 & 6 & 37.6 & 20.8 & 3522 & 63.5 & 6.01 & 5.72 & 5.98 \\
% % 47 & 6 & 4.32 & 6.7 & 38.3 & 21.5 & 3522 & 40.3 & 5.85 & 5.67 & 5.87 \\
% % 49 & 6.6 & 3.65 & 6.48 & 37.6 & 20.8 & 3522 & 55.8 & 5.95 & 6.08 & 5.84 \\
% % 50 & 6.3 & 3.32 & 5.88 & 37.3 & 20.5 & 3522 & 35.4 & 5.75 & 5.38 & 5.4 \\ 
% \hline\hline
% \end{tabular}
% \end{table}


==> authorlist.tex <==
%%%%% Please sign your name and affiliation below - in the format provided


%%% e.g. 
A. T. Barnes - Argelander-Institut f\"ur Astronomie, Universit\"at Bonn, Auf dem H\"ugel 71, 53121 Bonn, Germany 

%%% Please complete below.. 

L. Ubeda - Space Telescope Science Institute, Baltimore, MD 21218, USA 
B. Groves - International Centre for Radio Astronomy Research, The University of Western Australia, 35 Stirling Hwy, 6009 Crawley, WA, Australia
J.C. Lee - Gemini Observatory/NSF’s NOIRLab, 950 N. Cherry Avenue, Tucson, AZ, 85719, USA &
Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721
Francesco Belfiore, INAF— Osservatorio Astrofisico di Arcetri, Largo E. Fermi 5, I-50125, Florence, Italy
Médéric Boquien - Centro de Astronomía (CITEVA), Universidad de Antofagasta, Avenida Angamos 601, Antofagasta, Chile
Daniel A. Dale - Department of Physics \& Astronomy, University of Wyoming, Laramie, WY 82071 USA
Ralf S. Klessen - Universit\"at Heidelberg, Zentrum f\"ur Astronomie, Institut f\"ur Theoretische Astrophysik, Albert-Ueberle-Str.\ 2, 69120 Heidelberg, Germany  \& niversit\"{a}t Heidelberg, Interdisziplin\"{a}res Zentrum f\"{u}r Wissenschaftliches Rechnen, Im Neuenheimer Feld 225, 69120 Heidelberg, Germany
Adam K. Leroy - Department of Astronomy, The Ohio State University, 140 West 18th Avenue, Columbus, OH 43210, USA
Hsi-An Pan - Department of Physics, Tamkang University, No.151, Yingzhuan Road, Tamsui District, New Taipei City 251301, Taiwan
Thomas G. Williams - Max-Planck-Institut f\"{u}r Astronomie, K\"{o}nigstuhl 17, D-69117, Heidelberg, Germany
Enrico Congiu - Departamento de Astronoḿıa, Universidad de Chile, Camino del Observatorio 1515, Las Condes, Santiago, Chile
K. Grasha - ARC DECRA Fellow \& 
Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT 2611, Australia \&
ARC Centre of Excellence for All Sky Astrophysics in 3 Dimensions (ASTRO 3D), Australia   

Mattia C. Sormani - Universit\"{a}t Heidelberg, Zentrum f\"{u}r Astronomie, Institut f\"{u}r theoretische Astrophysik, Albert-Ueberle-Str. 2, 69120 Heidelberg, Germany

Cosima Eibensteiner - Argelander-Institut f\"ur Astronomie, Universit\"at Bonn, Auf dem H\"ugel 71, 53121 Bonn, Germany

Jakob den Brok - Argelander-Institut f\"ur Astronomie, Universit\"at Bonn, Auf dem H\"ugel 71, 53121 Bonn, Germany

J.~M.~Diederik Kruijssen - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, 69120 Heidelberg, Germany

Fabian Scheuermann - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, 69120 Heidelberg, Germany

Eric Emsellem - European Southern Observatory, Karl-Schwarzschild-Stra{\ss}e 2, 85748 Garching, Germany / Univ Lyon, Univ Lyon1, ENS de Lyon, CNRS, Centre de Recherche Astrophysique de Lyon UMR5574, F-69230 Saint-Genis-Laval France

Laura A. Lopez - Department of Astronomy, The Ohio State University, 140 West 18th Avenue, Columbus, OH 43210, USA

Hamid Hassani - 4-183 CCIS, University of Alberta, Edmonton, Alberta, T6G 2E1,
Canada

Kathryn Kreckel - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, D-69120 Heidelberg, Germany

Elizabeth J. Watkins - Astronomisches Rechen-Institut, Zentrum f\"{u}r Astronomie der Universit\"{a}t Heidelberg, M\"{o}nchhofstra\ss e 12-14, 69120 Heidelberg, Germany

Sinan Deger - TAPIR, California Institute of Technology, Pasadena, CA 91125, USA

==> scratch/scratch.tex <==
%--------------------------------------------------- 
\begin{table}
    \centering
    \caption{Properties of the galaxy sample. We show in rows the galaxy name, central right ascension~(RA) and declination~(Dec), inclination~($i$), position angle~(PA), morphological type (Morph.), distance (Dist.), effective radius ($R_\mathrm{eff}$), globally averaged metallicity ($12+\log(\mathrm{O/H})$), total mass of atomic gas ($M_\mathrm{HI}$), molecular gas ($M_\mathrm{H_{2}}$) and stars ($M_\star$), and global star formation rate~(SFR).}
    \label{tab:galprops}
    
    \begin{tabular}{ccc}
    \hline
    Galaxy & Unit & Value \\
    \hline
    Name & - & NGC1672 \\ 
    RA $(a)$ & $\mathrm{{}^{\circ}}$ & 71.427 \\ 
    Dec $(a)$ & $\mathrm{{}^{\circ}}$ & -59.247 \\ 
    $i$ $(b)$ & $\mathrm{{}^{\circ}}$ & 42.6 \\
    PA $(b)$ & $\mathrm{{}^{\circ}}$ & 134.3 \\
    Morphology $(c)$ & - & Sb \\
    Distance $(d)$ & $\mathrm{Mpc}$ & 19.4 \\
    $R_\mathrm{eff}$ $(e)$ & $\mathrm{kpc}$ & 3.4 \\
    Metallicity $(f)$ & 12+log(O/H) & 8.56 \\
    $M_\mathrm{HI}$ $(g)$ & log($\mathrm{M_{\odot}}$) & 10.2 \\
    $M_\mathrm{H2}$ $(h)$ & log($\mathrm{M_{\odot}}$) & 9.9 \\
    $M_\star$ $(i)$ & log($\mathrm{M_{\odot}}$) & 10.7 \\
    SFR $(i)$ & log($\mathrm{M_{\odot}\,yr^{-1}}$) & 0.9\\
    \hline
    \end{tabular}

    \begin{minipage}{\columnwidth}
    \small
    \vspace{1mm} References: 
    $(a)$ From \cite{Salo2015}.
    $(b)$ From \cite{Lang2020}, based on PHANGS \mbox{CO(2--1)} kinematics. 
    $(c)$ Morphological classification taken from HyperLEDA \citep{Makarov2014}.
    $(d)$ Source distances are taken from the compilation of \citet{Anand2021}. 
    % $(d)$ Source distances are taken from several sources, using different methods. ic5332, ngc2835, ngc5068 are from PHANGSTRGB, using the Tip of the Red Giant Branch (TRGB) method. ngc0628, ngc1365, ngc3351, ngc3627, are from \citet{Jacobs2009} also using the TRGB method. ngc1433, ngc1512 are determined using the PNLF method from PHANGSPNLF. ngc1087, ngc1566, ngc4303 use the Group method and are from \citet{Kourkchi2017}. ngc1300, ngc1385, ngc1672, ngc7496 are determined using the NAM method from \citet{Shaya2017} and \citet{Kourkchi2020}. ngc4254 is determined using the SCM from \citet{Nugent2006}. ngc4321, ngc4535 are determine using Cepheids from \citet{Freedman2001}.  
    $(e)$ $R_\mathrm{eff}$ that contains half of the stellar mass of the galaxy \citep{Leroy2021a}. 
    $(f)$ Averaged metallicity within the area mapped by MUSE, computed using the Scal method of \citet{Pilyugin2016}; see \citet{kreckel19} for more details. 
    $(g)$ Total atomic gas mass taken from HYPERLEDA \citep{Makarov2014}.
    $(h)$ Total molecular gas mass determined from PHANGS \mbox{CO(2--1)} observations (see \citealp{Leroy2021a}). 
    $(i)$ Derived by \citet{Leroy2021a}, using \textit{GALEX}~UV and \textit{WISE}~IR photometry, following a similar methodology to \cite{Leroy2019}.
    \end{minipage}
      
\end{table}

